A Tool for Reliability Assessment of Smart and Active Distribution Systems -- RELSAD

With increased penetration of new technology in the distribution systems such as renewable energy resources, flexible resources, and information and communication technology, the distribution systems become more complex and dynamic. The traditional reliability analysis methods do not consider the new components and technology and new considerations need to be taken to address these new changes in the distribution system. This paper presents an open-source reliability assessment tool for smart and active distribution systems (RELSAD). The tool aims to function as a foundation for reliability calculation in the smart and active distribution systems, where these new components and technologies are included. The tool is made as a Python package built up based on an object-oriented programming approach. The method will be illustrated on the IEEE 33-bus system with the inclusion of generation, battery, and ICT.

==> Sections/05Validation.tex <==
\section{Validation}
\label{validation}

The reliability data result is validated by comparing the result against reliability result of the \textit{Roy Billinton test system} (RBTS) bus 2 \cite{allan1991reliability}. The traditional reliability data for the RBTS bus 6 network is calculated analytically, and the reliability indices will be compared to the reliability indices obtained from the simulation tool. The result is illustrated in Tab \ref{tab:Validation}. The deviation is small with the highest number of X\%.  

\begin{table}[H]
    \caption{Comparison between analytical approach and the simulation tool}
    \center
\begin{tabular}{cccc} 
     \hline
     \textbf{Indices} & \textbf{Analytical}& \textbf{Simulation} & \textbf{Difference [\%]}\\ \hline
     
    \textbf{SAIFI}  & 0.248 & X & Y\\ 
    \textbf{SAIDI}  & 3.61 & X & Y\\ 
    \textbf{CAIDI}  & 14.55 & X & Y\\ 
    \textbf{ENS}  & 37746 & X & Y\\ \hline


\end{tabular}
\label{tab:Validation}
\end{table}
